PowerInfer: Fast Large Language Model Serving with a Consumer-grade GPU

This paper introduces PowerInfer, a high-speed Large Language Model (LLM) inference engine on a personal computer (PC) equipped with a single consumer-grade GPU. The key principle underlying the design of PowerInfer is exploiting the high locality inherent in LLM inference, characterized by a power-law distribution in neuron activation. This distribution indicates that a small subset of neurons, termed hot neurons, are consistently activated across inputs, while the majority, cold neurons, vary based on specific inputs. PowerInfer exploits such an insight to design a GPU-CPU hybrid inference engine: hot-activated neurons are preloaded onto the GPU for fast access, while cold-activated neurons are computed on the CPU, thus significantly reducing GPU memory demands and CPU-GPU data transfers. PowerInfer further integrates adaptive predictors and neuron-aware sparse operators, optimizing the efficiency of neuron activation and computational sparsity. The evaluation shows that PowerInfer significantly outperforms llama.cpp by up to 11.69x while retaining model accuracy across various LLMs (including OPT-175B) on a single NVIDIA RTX 4090 GPU. For the OPT-30B model, PowerInfer achieves performance comparable to that of a high-end server-grade A100 GPU, reaching 82% of its token generation rate on a single consumer-grade RTX 4090 GPU.

==> Makefile <==
DOC_NAME    := ms

PS2PDF      := ps2pdf14

#use the following options to avoid the embedded font problem.
DVIPS       := dvips -j0 -Ppdf -Pdownload35 -G0 -t letter -D 1200 -Z -mode ljfzzz
LATEX       := pdflatex
FIG2DEV     := fig2dev

#use the following options to generate into a single html.
LATEX2HTML  := latex2html -split 0 -split +0 -link 0 -no_navigation -no_footnode -show_section_numbers -local_icons
DOXYGEN     := doxygen
BIBTEX	    := bibtex

BASE := Makefile $(wildcard *.tex) $(wildcard *.bib)
BASE := $(BASE) $(wildcard ./pic/*.eps)

PSOPT 	:=  -dNOPAUSE -dBATCH \
	-sDEVICE=pdfwrite -dPDFSETTINGS=/prepress\
	-dCompatibilityLevel=1.5 \
	-dCompressPages=true -dUseFlateCompression=false \
	-sPAPERSIZE=letter \
	-dSubsetFonts=true -dEmbedAllFonts=true \
	-dProcessColorModel=/DeviceGray \
	-dDetectBlends=true -dOptimize=true \
	-dDownsampleColorImages=true -dColorImageResolution=1200 \
	-dColorImageDownsampleType=/Average -dColorImageFilter=/FlateEncode \
	-dAutoFilterColorImages=false -dAntiAliasColorImages=false \
	-dColorImageDownsampleThreshold=1.50000 \
	-dDownsampleGrayImages=true -dGrayImageResolution=1200 \
	-dGrayImageDownsampleType=/Average -dGrayImageFilter=/FlateEncode \
	-dAutoFilterGrayImages=false -dAntiAliasGrayImages=false \
	-dGrayImageDownsampleThreshold=1.50000 \
	-dDownsampleMonoImages=true -dMonoImageResolution=1200 \
	-dMonoImageDownsampleType=/Average -dMonoImageFilter=/FlateEncode \
	-dAutoFilterMonoImages=false -dAntiAliasMonoImages=false \
	-dMonoImageDownsampleThreshold=1.50000

all: pdf

pdf: $(DOC_NAME).pdf

%.pdf: %.ps
	$(PS2PDF) $(PSOPT) $< $@
	@cat $(DOC_NAME).log | grep Warning

%.ps: %.dvi
	$(DVIPS) $< -o $@

%.dvi: $(BASE)
	@make clean
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex

html: $(DOC_NAME)/$(DOC_NAME).html

%.html: $(BASE)
	@rm -rf $(DOC_NAME)
	$(LATEX2HTML) $*.tex

clean:
	@rm -rf $(DOC_NAME).pdf $(DIFF_NAME).pdf *.ps *.dvi *.aux *.log *.bbl  *.blg *.idx *.out *~ pic/*~ $(DOC_NAME)

.PHONY: clean all pdf html

### Makefile ends here

